JoyAI-Voice 2.0: A Full-Continuous Autoregressive Speech Generation Model with Semantic-Acoustic Joint Representation

We present JoyAI-Voice~2.0, an end-to-end anthropomorphic speech generation model built upon a fully continuous, dual-encoder architecture. Raw speech is encoded into continuous latents and partitioned into patches. Each patch is decomposed by a semantic-acoustic dual encoder into a semantically purified representation and an acoustic representation, which are fused and jointly fed to a causal autoregressive Transformer for planning. The Transformer predicts the conditioning for the next patch, and a local diffusion Transformer renders its full latents for 48\,kHz synthesis. The model is trained with a joint flow-matching and stop-prediction objective, followed by supervised fine-tuning and reinforcement learning with DiffusionNFT to improve model performance. It achieves the lowest average word error rate of 2.51\% on Seed-TTS, a 14.9\% relative reduction over the strongest baseline, and state-of-the-art attribute fidelity on InstructTTSEval in both Chinese and English, leading on 5 of 10 perceptual dimensions with the highest overall score of 0.893 on MDVD-Eval.

==> sections/022_datapipeline.tex <==
\section{Data Pipeline} @nihao
\label{sec:datapipeline}

==> sections/033_acceleration.tex <==
\section{Inference Efficiency} 
\label{sec:acceleration}

JoyAI-Voice 2.0 combines an autoregressive backbone with a patch-wise audio side path. Its primary inference bottleneck arises not from a single compute-intensive operator, but from repeated execution of the audio branch across patches. Each patch launches  thousands of small kernels, incurring substantial host-side dispatch overhead and device-side kernel fragmentation. We address these bottlenecks with four complementary optimizations: (i) incremental KV caching to reuse historical context and avoid redundant computation across patches; (ii) CUDA Graph capture of audio-branch stages to reduce host-side dispatch overhead; (iii) capacity-bucketed cross-request batching to improve GPU utilization; and (iv) compiler-level operator fusion to reduce kernel fragmentation.
